Spatially Structured Regression for Non-conformable Spaces: Integrating Pathology Imaging and Genomics Data in Cancer

The spatial composition and cellular heterogeneity of the tumor microenvironment plays a critical role in cancer development and progression. High-definition pathology imaging of tumor biopsies provide a high-resolution view of the spatial organization of different types of cells. This allows for systematic assessment of intra- and inter-patient spatial cellular interactions and heterogeneity by integrating accompanying patient-level genomics data. However, joint modeling across tumor biopsies presents unique challenges due to non-conformability (lack of a common spatial domain across biopsies) as well as high-dimensionality. To address this problem, we propose the Dual random effect and main effect selection model for Spatially structured regression model (DreameSpase). DreameSpase employs a Bayesian variable selection framework that facilitates the assessment of spatial heterogeneity with respect to covariates both within (through fixed effects) and between spaces (through spatial random effects) for non-conformable spatial domains. We demonstrate the efficacy of DreameSpase via simulations and integrative analyses of pathology imaging and gene expression data obtained from $335$ melanoma biopsies. Our findings confirm several existing relationships, e.g. neutrophil genes being associated with both inter- and intra-patient spatial heterogeneity, as well as discovering novel associations. We also provide freely available and computationally efficient software for implementing DreameSpase.

==> definitions.tex <==
\newcommand{\vb}[1]{\textcolor{magenta}{\textsf{[#1]}}}
\newcommand{\no}[1]{\textcolor{red}{\textsf{[#1]}}}
\newcommand{\redacted}[1]{\textcolor{red}{\textsf{[#1]}}}
\newcommand{\jk}[1]{\textcolor{violet}{\textsf{[JK: #1]}}}
\newcommand{\jkedit}[1]{
\textcolor{violet}{#1}
}
\newcommand{\tempsupref}[1]{\textcolor{red}{\textsf{[#1]}}}
\newcommand{\todo}[1]{\textcolor{red}{\textsf{[TODO: #1]}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My commands
\newcommand{\bs}[1]{{\boldsymbol{#1}}}
\renewcommand{\epsilon}{\varepsilon}

\newcommand{\normdens}[3]{\frac{1}{\sqrt{2\pi #1^2}}\exp\left(\frac{1}{2 #1^2}(#2 - #3)^2\right)}

\newcommand{\mvcardenskern}[3]{\text{det}\left( #1 \left[D_w(\bm{W}_i) - #2 \bm{W}_i\right]^{-1} \right)^{-1/2} \exp\left(-\frac{1}{2}\left({#3}^T  \left[ #1 \left[D_w(\bm{W}_i) - #2 \bm{W}_i\right]^{-1} \right] #3 \right)\right)}

\newcommand{\normdenszero}[2]{\frac{1}{\sqrt{2\pi #1^2}}\exp\left(\frac{-1}{2 #1^2}#2^2\right)}

\newcommand{\normdenszeroprop}[2]{\exp\left(\frac{-1}{2 #1^2}#2^2\right)}

\newcommand{\mvnormdenszero}[3]{\text{det}\left( #1 \right)^{-1/2} \exp\left(-\frac{1}{2}\left\{{#2}^T \left[ #1 \right]^{-1} #2\right\}\right)}

\newcommand{\mvnormdenszerobr}[3]{\text{det}\left( #1 \right)^{-1/2} \\ &\exp\left(-\frac{1}{2}\left({#2}^T \left[ #1 \right]^{-1} #2\right)\right)}

\newcommand{\var}{\text{var}}

\newcommand{\itmethodname}{\texttt{DreameSpase}}
\newcommand{\methodname}{DreameSpase}
\newcommand{\itmethodnames}{\texttt{DreameSpase} }
\newcommand{\methodnames}{DreameSpase }
